VisRL: Intention-Driven Visual Perception via Reinforced Reasoning

Visual understanding is inherently intention-driven - humans selectively focus on different regions of a scene based on their goals. Recent advances in large multimodal models (LMMs) enable flexible expression of such intentions through natural language, allowing queries to guide visual reasoning processes. Frameworks like Visual Chain-of-Thought have demonstrated the benefit of incorporating explicit reasoning steps, where the model predicts a focus region before answering a query. However, existing approaches rely heavily on supervised training with annotated intermediate bounding boxes, which severely limits scalability due to the combinatorial explosion of intention-region pairs. To overcome this limitation, we propose VisRL, the first framework that applies reinforcement learning (RL) to the problem of intention-driven visual perception. VisRL optimizes the entire visual reasoning process using only reward signals. By treating intermediate focus selection as an internal decision optimized through trial-and-error, our method eliminates the need for costly region annotations while aligning more closely with how humans learn to perceive the world. Extensive experiments across multiple benchmarks show that VisRL consistently outperforms strong baselines, demonstrating both its effectiveness and its strong generalization across different LMMs. Our code is available at https://github.com/zhangquanchen/VisRL.

==> Sec/related_long.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{Multi-modal Large Language Models}
With the advancement of large language models (LLMs)~\cite{llm:radford2018improving,llm:radford2019language,llm0:floridi2020gpt,llm1:few-shot,llm10:bi2024deepseek,llm11:cai2024internlm2,llm12:jiang2024identifying,llm2:zhang2022opt,llm3:touvron2023llama,llm4:touvron2023llama,llm5:bai2023qwen,llm6:team2023internlm,llm7:almazrouei2023alghafa,llm8:glm2024chatglm,llm9:yang2023baichuan}, multi-modal large language models which integrate vision and language modalities have also experienced rapid development. This progress enables AI systems to better perceive and understand the real-world interplay between visual and textual information. Notable methods like LLaVA~\cite{mllm:liu2023llava} align image tokens with pre-trained LLMs by training a projector, while other approaches utilize a Q-Former~\cite{li2022blip,li2023blip} to learn image embeddings via learnable queries after extracting image features. Generally, the training paradigm of recent LMMs~\cite{mllm:beyer2024paligemma,mllm:chen2024internvl,mllm:hu2024minicpm,mllm:li2024llava,mllm:liu2023improvedllava,mllm:liu2024llavanext,mllm:liu2023llava,mllm:lu2024deepseek,mllm:wang2024qwen2,mllm:wu2024deepseek,mllm:zhang2024internlm} consists of three stages: (1) Pre-training, which aligns image tokens with the LLM’s representation space using large-scale image-text pairs; (2) Instruction fine-tuning, which enhances task performance and instruction adherence through diverse training data; and (3) Alignment, which employs reinforcement learning to align the model with human values or specific constraints (e.g. minimizing hallucinations). Moreover, the utility of LMMs has broadened across a multitude of domains, such as video understanding~\cite{video1,video2,video3}, fine-grained localization~\cite{fg-l1,fg-l2,fg-l3}, and image generation~\cite{ig1,ig2}.


\paragraph{Intention-Driven Visual Models}
% \todo{visual cot, v star, ...}
Recently, several methods have attempted to enhance models' intention-driven visual perception capabilities. VisCoT~\cite{shao2024visual} employs a multi-turn interpretable processing mechanism with \emph{bounding boxes} that dynamically focus on visual inputs. Similarly, SpatialCoT~\cite{rela:liu2025spatialcot} achieves spatial grounding through \emph{spatial coordinates}, while SegLLM~\cite{rela:wang2024segllm} leverages \emph{mask-labeled} data to enable reasoning about complex user segmentation intentions. V* (SEAL)~\cite{rela:vstar} provides an LLM-guided search mechanism for efficient visual querying. Besides, both MLLM-TPO~\cite{rela:tpo} and VisionLLM v2~\cite{rela:wu2025visionllmv2} achieve intention-driven perception by training decoders for specific downstream tasks. Additionally, MVoT ~\cite{rela:mvot}introduces a text-image-text reasoning paradigm by training on interleaved data. However, these methods heavily rely on dense-labeled data (e.g., bounding boxes, spatial coordinates, masks, multi-round reasoning conversations), which constrains their ability to scale further.

On the other hand, several methods employ tool-usage for enhancement. Specifically, AURORA~\cite{rela:aurora} leverages specialized detection models, while Plug-and-Play~\cite{rela:plugandplay} adopts a multi-agent framework. Besides, ViRReq~\cite{rela:virreq} leverages the knowledge base to decompose visual recognition. However, these approaches do not fundamentally enhance the intrinsic capabilities of the models themselves.

We propose a novel approach that does not rely on dense-labeled data for training. Instead, VisRL leverages RL to learn intelligent visual perception abilities from task feedback.

\paragraph{Multimodal Models with Chain-of-Thoughts}
Some methods focus on enhancing visual reasoning capabilities via Chain-of-Thoughts (CoT), thus achieve stronger visual perception ability. The methods can be broadly categorized into two types: (1) Text-thought methods: ~\cite{rela_new:r1v, rela_new:llamavo1,rela_new:alignanything,rela_new:openrlhf}
elicit textual CoT reasoning of LLMs in visual reasoning tasks by introducing RL method inspired by~\cite{rela:deepseekr1}, ultimately guiding towards the final response. (2) Multi-modal-thought methods: the Mind’s Eye~\cite{rela_new:mideye} elicit spatial reasoning of LLMs by visualizing their reasoning traces. Besides, Insight-V~\cite{rela:insight-v} adopts a long-chain visual reasoning approach to derive answers, while VISCO~\cite{rela:wu2024visco} incorporates a critique-based self-improvement mechanism for visual reasoning. Additionally, ~\cite{rela:liu2025spatialcot,shao2024visual,rela:wang2024segllm} first generate visual marks (e.g. bounding boxes, spatial coordinates, masks), and subsequently perform CoT reasoning based on these fine-grained visual marks. 
% \todo{type1: text thoughts. r1v, open-r1-multimodal, align-anything, openrlhf-m, LlamaV-o1, ...}

% \todo{type2: multimodal thoghts. SpatialCoT, visual cot, Mind’s Eye of LLMs, SegLLM, ...}
